nach0: Multimodal Natural and Chemical Languages Foundation Model

Large Language Models (LLMs) have substantially driven scientific progress in various domains, and many papers have demonstrated their ability to tackle complex problems with creative solutions. Our paper introduces a new foundation model, nach0, capable of solving various chemical and biological tasks: biomedical question answering, named entity recognition, molecular generation, molecular synthesis, attributes prediction, and others. nach0 is a multi-domain and multi-task encoder-decoder LLM pre-trained on unlabeled text from scientific literature, patents, and molecule strings to incorporate a range of chemical and linguistic knowledge. We employed instruction tuning, where specific task-related instructions are utilized to fine-tune nach0 for the final set of tasks. To train nach0 effectively, we leverage the NeMo framework, enabling efficient parallel optimization of both base and large model versions. Extensive experiments demonstrate that our model outperforms state-of-the-art baselines on single-domain and cross-domain tasks. Furthermore, it can generate high-quality outputs in molecular and textual formats, showcasing its effectiveness in multi-domain setups.

==> parts/chem_llm_related.tex <==
\subsection{Language Models in Chemistry}

LMs have a long history of research and application in the fields of chemistry and drug discovery. In particular, a widely utilized molecular representation called SMILES allows to work with molecules in a string format. 

The CharRNN \citep{segler2018charnn} architecture generates molecule as a sequence of SMILES tokens and can be trained to model the unconditional molecular distribution by maximizing the log likelihood of the training data. The RNN architecture can be used as decoder or/and encoder part in a variational autoencoder framework (VAE)  to learn meaningful latent space. Moreover, SMILES-based LMs can be further utilized in Reinforcement Learning \citep{zhavoronkov2019deep} and Gaussian Processes \citep{gomezbombarelli2018automatic} algorithms to optimize molecular properties and find novel molecular structures that satisfy chemical constraints.

MolMIM \citep{reidenbach2022improving} is a latent-space Mutual Information Machine (MIM) model \citep{livne_2020} designed for molecules. 
The model learns to embed tokenized SMILES into an informative and clustered continuous latent space. 
MolMIM has demonstrated to be very useful in the controlled generation of small molecules given one or more score functions.

Inspired by the recent advancements of Transformer-like architectures in NLP \citep{vaswani2017attention}, the drug discovery community has adopted best practices in the field of molecular generation, e.g., LM-based models such as MolBERT, ChemGPT, T5Chem, MolFolrmer, Chemformer, BARTSmiles \citep{fabian2020molecular,frey2022neural,lu2022unified,ross2022molformer,irwin2022chemformer,chilingaryan2022bartsmiles}

Molecular Transformer \citep{schwaller2019moleculartransformer} utilizes seq2seq Transformer \citep{vaswani2017attention} language model and trained to predict reactions outcomes. It takes SMILES representation of reactant and reagents and tries to predict SMILES of reaction result. 

The Chemformer architecture \citep{irwin2022chemformer} is based on BART  \citep{lewis2020bart} and utilizes a dataset of 100 million SMILES from the ZINC-15 dataset \citep{sterling2015zinc15} for pretraining. The pretrained model is subsequently fine-tuned for various downstream tasks including reaction and property prediction. The pretraining and downstream tasks specifically focus on chemical datasets. The Chemformer vocabulary is constructed using regular expression matching on canonical SMILES, resulting in a total of 523 tokens, with 250 tokens specifically representing chemical entities identified through the regular expression matching process.

Similar to Chemformer \citep{irwin2022chemformer}, T5Chem \citep{lu2022unified} is also pretrained from scratch with a chemical vocabulary on a dataset of 97 millions of molecules from Pubchem. T5Chem is built upon the T5 architecture \citep{raffel2020exploring}. The maximum vocabulary size was set to 100, which includes 70 tokens from character-level tokenization of SMILES, five special structural tokens (s, /s, unk, pad, mask), six prompting tokens, and 19 placeholders. Downstream tasks contains reactions prediction subtasks. We note that both Chemformer and T5Chem do not include tokens for natural language texts.
%The model can be accessed via \url{https://github.com/HelloJocelynLu/t5chem}.

The MolFormer model \citep{ross2022molformer} also focuses only on chemical tasks. On the pretraining stage, the model handles 1.1 billion of molecules, consisting of 1 billion from ZINC and 111 millions from PubChem. Finetuning is performed on a set of classification and regression molecular prediction tasks from MoleculeNet \citep{wu2018moleculenet}. The vocabulary of MolFormer contains 2362 tokens covering string fragments found by regular expressions.

Another T5-based architecture is MolT5 \citep{edwards2022translation}. In contrast with T5Chem \citep{lu2022unified}, this model is pre-trained on both chemical and NLP data and tasks - the large C4 corpus and 100 million SMILES strings from ZINC15 \citep{sterling2015zinc15} used in Chemformer \citep{irwin2022chemformer}. The model is further fine-tuned on the ChEBI-20 dataset \citep{edwards2021text2mol}, which consists of molecule-description pairs.

Galactica \citep{taylor2022galactica} large language model trains on data from multiple domains, including scientific corpus of papers, knowledge bases, equations, code and others. What matter for us, Galactica incorporate several sources with chemical data - publications with chemical entities, chemical compounds, chemical reactions, chemical properties predictions. To represent SMILES formulas, Galactica utilizes character-based tokenization and encloses the sequences with {\tt [START\_SMILES]} and {\tt [END\_SMILES]} tags.


%Chemformer
%T5chem
%MolT5
%Galactica
%MolFormer

%https://www.nature.com/articles/s42256-022-00580-7 -- pdf of this %work is transformer channel


==> parts/related.tex <==
\section{Related Work}
\subsection{Language Models}

Self Supervised Learning is an emerging area of research in machine learning that has received significant attention in recent years. Self Supervised Learning techniques aim to enable deep learning models to learn from unlabeled data by creating their own labels through a pre-defined objective.  
A number of LMs has been proposed for the biomedical and clinical domain, e.g., BioBERT, BioGPT, GatorTron, BioBART \citep{lee2020biobert,phan2021scifive,luo2022biogpt,yang2022gatortron,yuan2022biobart}.
%see a list of publcily available checkpoints at \url{https://huggingface.co/spaces/hf-ml4h/biomedical-language-models}. 
\cite{shin2020biomegatron} studied BERT-based BioMegatron model and several factors that can affect performance, such as the sub-word vocabulary set, model size, pre-training corpus, and domain transfer. They found that the subword vocabulary is the most critical factor, while larger model size does not necessarily translate to better performance.
%Foundation models build upon the concept of SSL by pretraining a single model over unlabeled data that can be easily adapted to any task \citep{bommasani2021opportunities}. 
LLMs are considered to be the most effective and adaptable foundation models due to rich supervision contained within raw text data. Surprisingly, training with LLMs and vast amounts of data resulted in impressive outcomes such as generalization, multi-tasking, zero-shot and few-shot model capabilities \citep{radford2019language,brown2020language,kojima2022large}. 
Recent studies have investigated these key capabilities of models across biomedical NLP tasks \citep{phan2021scifive,fries2022bigbio,parmar2022boxbart}. 

\cite{phan2021scifive} introduced SciFive, a domain-specific T5 model \citep{raffel2020exploring}, pre-trained on PubMed abstracts and PMC articles and fine-tuned on 14 BioNLP datasets. The model performed on par with single-task BERT and outperformed the latter on classification and text generation tasks, respectively. \cite{parmar2022boxbart} fine-tuned the BART (base) model \citep{lewis2020bart} on a collection of 32 instruction-based tasks for biomedical NLP. This model outperforms single-task baseline and multi-task baseline without instructions by 3\% and 18\%, respectively. 
\cite{fries2022bigbio} trained a single encoder-only BioLinkBERT-base \citep{yasunaga2022linkbert} model with a separate classification head for 107 tasks of a BigBio library. The model performs markedly worse than single-task BioLinkBERT model, with differences between 1.5 and 11.2 percentage points of F1. Zero-shot evaluation showed that T5 and GPT model families (e.g., SciFive base/large \citep{phan2021scifive}, T5-v1.1-xxl \citep{raffel2020exploring}) often fail to generalize to biomedical text.

Table \ref{tab:comparison} provides comparison with existing encoder-decoder models.
 
\begin{table}
\caption{Comparison with existing encoder-decoder models. The column ``NL texts'' specifies whether the model was pretrained on natural language (NL) texts, while the column  ``chem. data'' indicates whether the model was pretrained on chemistry. The column ``specialized tokens'' indicate if the model utilizes specialized tokenization for chemical data.} \label{tab:comparison}
\begin{tabular}{p{1.6cm}|p{1.5cm}p{1.5cm}|p{1.0cm}p{1.0cm}p{1.0cm}|p{1.8cm}}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{pre-training}} & \multicolumn{3}{c|}{\textbf{tasks on the fine-tuning stage}} &  \\ %\hline
 & NL texts & chem. data & NLP  & chem. & cross-domain & specialized chem. tokens \\ \hline
FLAN & \cmark  & \xmark & \cmark & \xmark & \xmark & \xmark \\ %\hline
SciFive & \cmark  & \xmark & \cmark & \xmark & \xmark & \xmark \\ %\hline
Chemformer & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark  \\ %\hline
MolFormer & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark  \\ %\hline
T5Chem & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark  \\ %\hline
MolT5 & \cmark  & \cmark & \xmark & \xmark & \cmark & \xmark \\ %\hline
Galactica & \cmark  & \cmark & \cmark  & \cmark & \xmark & \cmark \\ %\hline
Our & \cmark  & \cmark & \cmark  & \cmark & \cmark  & \cmark \\ \hline
\end{tabular}
\end{table}

%https://academic.oup.com/bib/article-abstract/23/6/bbac409/6713511

\input{parts/chem_llm_related}

